Convergence Analysis of Sequential Split Learning on Heterogeneous Data

Federated Learning (FL) and Split Learning (SL) are two popular paradigms of distributed machine learning. By offloading the computation-intensive portions to the server, SL is promising for deep model training on resource-constrained devices, yet still lacking of rigorous convergence analysis. In this paper, we derive the convergence guarantees of Sequential SL (SSL, the vanilla case of SL that conducts the model training in sequence) for strongly/general/non-convex objectives on heterogeneous data. Notably, the derived guarantees suggest that SSL is better than Federated Averaging (FedAvg, the most popular algorithm in FL) on heterogeneous data. We validate the counterintuitive analysis result empirically on extremely heterogeneous data.

==> sections/relateds.tex <==
\section{Additional related work}\label{sec:appendix:additional related work}
\paragraph{Variants of SL.} SL is deemed as a promising paradigm for distributed model training at resource-constrained devices, given its computational efficiency on the client side. Most existing works focus on reducing the training delay arising from the relay-based training manner in the multi-user scenario. \texttt{SplitFed} \citep{thapa2020splitfed} is one popular model parallel algorithm that combines the strengths of FL and SL, where each client has one corresponding instance of server-side model in the \textit{main server} to form a pair. Each pair constitutes a complete model and conducts the local update in parallel. After each training round, the \textit{fed server} collects and aggregates on the clien-side local updates. The aggregated client-side model will be disseminated to all the clients before next round. The \textit{main server} does the same operations to the instances of the server-side model. However, in \texttt{SplitFed}, the \textit{main server} is required for great computing power to support the multiple instances of server-side model. To address this issue, \cite{thapa2020splitfed} proposed \texttt{SplitFedv2}. The only change in \texttt{SplitFedv2} is that only one server-side model in \textit{main server}. So the server-side model has to process the activations (or smashed data) of the client-side model in sequence. The model gets updated in every single forward-backward propagation, which means that the server-side model makes more updates than the client-side model. The main point of \texttt{SplitFedv3} \citep{gawali2020comparison} is substituting alternative client training with alternative the mini-batch training. In vanilla SL, the local model makes one or more training passes over the local dataset (alternative client training). This may cause ``catastrophic forgetting'' issue \citep{gawali2020comparison, duan2022combined}. So \texttt{SplitFedv3} propose to use alternate mini-batch training, where a client updates its client-side model on one mini-batch, after which the client next in order takes over \citep{gawali2020comparison}, to mitigate the issue. \texttt{SFLG} \citep{gao2021evaluation} is one generalized variants of \texttt{SplitFed}. The clients are allocated to multiple groups. There is one server in each group. The training inside the group is identical to \texttt{SplitFedv2}. Then the server-side ``global'' models per group are aggregated (e.g., weighted averaging) to obtain the server-side global model of all groups. \texttt{FedSeq} \citep{zaccone2022speeding} is the same as \texttt{SFLG} except that the training inside the group is identical to vanilla SL. More variants can be found in \cite{thapa2021advancements, duan2022combined}.


\paragraph{Convergence analysis of SL.} The convergence analysis of SL is identical to standard Minibatch-SGD on IID data \citep{wang2022fedlite,park2021communication}, so some convergence properties of Minibatch SGD is applied to SL too. The algorithm in \cite{han2021accelerating} reduces the latency and downlink communication on \texttt{SplitFed} by adding auxiliary networks at client-side to generate the local loss for model updating. Their convergence analysis combines the analysis of \cite{belilovsky2020decoupled} and \texttt{FedAvg}. \cite{wang2022fedlite} proposed \texttt{FedLite} to reduce the uplink communication overhead by compressing activations with product quantization and provided the convergence analysis of \texttt{FedLite}. However, their convergence recovers that of Minibatch SGD when there is no quantization. SGD with biased gradients \citep{ajalloeian2020convergence} is also related. However, it only converges to a neighborhood of the solution. Furthermore, we find that \cite{woodworth2020local, woodworth2020minibatch} compared the convergence of distributed Minibatch SGD and local SGD under homogeneous and heterogeneous settings. To differentiate our work, we show how Minibatch SGD, FL and SL operate in Table~\ref{table:comparisons of operate way}. They all aim to optimize one global objective, $\min f(\rvx) = \frac{1}{N} \sum_{i=1}^N f_i(\rvx)$ for $N$ clients, each of which has its own local dataset $\gD_i$. Here $f_i(\rvx) \coloneqq \E_{\xi_i \sim \gD_i}[f_i(\rvx; \xi_i)]$ is the local objective function of client $i$. The learning rate is denoted as $\eta$. The global model parameter is denoted as $\rvx^r$ in the $r$-th round. In particular, we use $\rvx_i^{(r,k)}$ to denote the local model parameter of client $i$ after $k$-th local update in the $r$-th round for FL and SL. We use $\nabla f_i(\rvx;\xi)$ to represent the stochastic gradient of $f_i$ computed by the parameter $\rvx$ and the data sample $\xi$. Note that we assume that the number of local update steps of all clients in FL and SL is $K$. We can see that (i) there is no local update and each client computes $K$ stochastic gradients at the same point $\rvx^r$ in Minibatch SGD; (ii) clients in FL make local training in parallel, while clients in SL make local training in sequence.


\begin{table}[ht]
	%\tabcolsep=0.12cm
	\renewcommand{\arraystretch}{1.6}
	\centering
	\caption{The update rules of Minibatch SGD, FL (Local SGD) and SL.}
	\label{table:comparisons of operate way}
	\begin{scriptsize}
		\begin{tabular}{cll}
			\hline\hline
			Algorithm  &Global model update &Local update of client $i$\\
			\midrule
			\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Minibatch \\ SGD \end{tabular}}
			&\multirow{2}{*}{
				\(\displaystyle
				\rvx^{r+1} = \rvx^{r} - \eta \frac{1}{NK}\sum_{i=1}^{N}\sum_{k=0}^{K-1} \nabla f_i (\rvx^r;\xi_{i}^{(r,k)})
				\)} &-\\
			& &-\\ \hline
			\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Local SGD \\(or FL) \end{tabular}}
			&\multirow{2}{*}{
				\(\displaystyle
				\rvx^{r+1} = \rvx^{r} - \eta\frac{1}{N}\sum_{i=1}^{N}\sum_{k=0}^{K-1} \nabla f_i (\rvx_{i}^{(r,k)};\xi_{i}^{(r,k)}) \)}
			&Initialize: $\rvx_i^{(r,0)} = \rvx^r$ \\
			& &Update: $\rvx_i^{(r,k+1)} = \rvx_i^{(r,k)} - \eta \nabla f_i(\rvx_{i}^{(r,k)};\xi_{i}^{(r,k)})$ \\ \hline
			\multirow{2}{*}{SL} 
			&\multirow{2}{*}{
				\(\displaystyle
				\rvx^{r+1} = \rvx^{r} - \eta\sum_{i=1}^{N}\sum_{k=0}^{K-1} \nabla f_i (\rvx_{i}^{(r, k)};\xi_{i}^{(r,k)}) \)}
			&Initialize: $\rvx_i^{(r,0)} = \rvx_{i-1}^{(r,K)}$\\
			& &Update: $\rvx_i^{(r,k+1)} = \rvx_i^{(r,k)} - \eta \nabla f_i(\rvx_{i}^{(r,k)};\xi_{i}^{(r,k)})$ \\
			\hline\hline
		\end{tabular}
	\end{scriptsize}
\end{table}



